Empirical Bayesian Approaches for Robust Constraint-based Causal Discovery under Insufficient Data

Causal discovery is to learn cause-effect relationships among variables given observational data and is important for many applications. Existing causal discovery methods assume data sufficiency, which may not be the case in many real world datasets. As a result, many existing causal discovery methods can fail under limited data. In this work, we propose Bayesian-augmented frequentist independence tests to improve the performance of constraint-based causal discovery methods under insufficient data: 1) We firstly introduce a Bayesian method to estimate mutual information (MI), based on which we propose a robust MI based independence test; 2) Secondly, we consider the Bayesian estimation of hypothesis likelihood and incorporate it into a well-defined statistical test, resulting in a robust statistical testing based independence test. We apply proposed independence tests to constraint-based causal discovery methods and evaluate the performance on benchmark datasets with insufficient samples. Experiments show significant performance improvement in terms of both accuracy and efficiency over SOTA methods.

==> tb_RAI_application.tex <==
%% RAI improvement application on UCI
\begin{table}[h!]
%\begin{wraptable}{r}{0.54\textwidth}
%\vspace*{-0.6\baselineskip}
	\caption{Predictive performance with BN classifier}
	%\vspace*{-0.6\baselineskip}
  \label{tb:applicationRAI}
  \centering
  %\renewcommand{\arraystretch}{0.95}% Tighter
  \scalebox{0.95}{
  %\begin{adjustbox}{width=,center}
  \begin{tabular}{|c|ccc|}
    \hline
    \hline
    %&&&&\\[-0.9em]
    %\multicolumn{2}{c|}{}&&&&\\[-1em]
    %\multicolumn{2}{c|}{STMB}
    \multirow{2}{*}{Dataset} &\multicolumn{3}{c|}{\underline{F1-score}}\\
    &$rI^{eB}$ & $rBF_{chi2}$ & RAI-BF \\ 
    %&&&&\\[-1em]
    \hline
    %&&&\\[-0.8em]
    Breast  &\textbf{0.87} &  0.79&0.62\\
    %&&&&\\[-1em]
    Congress  &\textbf{0.94} &0.90 & 0.86\\
    %&&&&\\[-1em]
    Heart  &0.75 &\textbf{0.76} &0.53 \\
    %&&&&\\[-1em]
    Parkinsons  &0.61 &\textbf{0.70} &0.38 \\
    %&&&&\\[-1em]
    Spect  &\textbf{0.59}  &0.58 &0.57 \\
    \hline
  \end{tabular}}
  %\end{adjustbox}
  %\vspace{-0.4cm}
\end{table}
%\vspace*{-\baselineskip}
%\end{wraptable}

==> tb_STMB_application.tex <==
%% STMB improvement application on UCI
%\begin{wraptable}{r}{0.54\textwidth}
%\vspace*{-0.8\baselineskip}
\begin{table}[h!]
    \caption{Predictive performance of MB discovery}
    %\vspace*{-0.6\baselineskip}
  \label{tb:applicationSTMB}
  \centering
  %\renewcommand{\arraystretch}{0.9}% Tighter
  \scalebox{0.95}{
  \begin{tabular}{|c|ccc|}
    \hline
    \hline
    &\multicolumn{3}{c|}{\underline{F1-score/Compression Rate}}\\%&\multicolumn{3}{c|}{Compression Rate}\\
    Dataset&$sI^{eB}$  & $sBF_{chi2}$ & STMB\\ %&$sI^{fB}$  & $sBF_{chi2}$ & STMB \\ 
    \hline
    Breast  & --/-- & 0.92/\textbf{0.37} & \textbf{0.93}/0.81\\ %& -- & \textbf{0.37} & 0.81\\
    Congress &\textbf{0.95}/\textbf{0.06} &\textbf{0.95}/\textbf{0.06}& 0.94/0.56\\ %&\textbf{0.06}&\textbf{0.06}&0.56\\
    Heart  & 0.77/\textbf{0.08} &\textbf{0.86}/0.21& 0.80/0.97\\
    %& \textbf{0.08} &0.21&0.97\\
    Parkinsons  & 0.59\textbf{0.04} & \textbf{0.83}/0.38& 0.79/0.95\\
    %& \textbf{0.04} & 0.38& 0.95\\
    Spect  & 0.72\textbf{0.68} &\textbf{0.74}/0.73 & 0.71/0.74\\
    %& \textbf{0.68} &0.73& 0.74\\
    \hline
  \end{tabular}}
%\vspace*{-\baselineskip}
\end{table}
%\end{wraptable}

==> tb_datasetinfo.tex <==
\begin{table*}[h!]
	\caption{\textcolor{red}{ADDED: Benchmark Classification Dataset Information}}
  \label{tb:datasetsinfo}
  \centering
  \scalebox{0.8}{
  \begin{tabular}{|c|c|c|c|c|}
    \hline
    \hline
    Dataset & number of samples for classes \\ 
    \hline
 Breast& \textcolor{red}{Better to draw figures instead of tables?}\\
 Congress & \\
 Heart & \\
 Parkinsons & \\
 Spect & \\
 & \textcolor{red}{Other?}\\
    \hline
  \end{tabular}}
\end{table*}
